Improving the Behaviour of Vision Transformers with Token-consistent Stochastic Layers

We introduce token-consistent stochastic layers in vision transformers, without causing any severe drop in performance. The added stochasticity improves network calibration, robustness and strengthens privacy. We use linear layers with token-consistent stochastic parameters inside the multilayer perceptron blocks, without altering the architecture of the transformer. The stochastic parameters are sampled from the uniform distribution, both during training and inference. The applied linear operations preserve the topological structure, formed by the set of tokens passing through the shared multilayer perceptron. This operation encourages the learning of the recognition task to rely on the topological structures of the tokens, instead of their values, which in turn offers the desired robustness and privacy of the visual features. The effectiveness of the token-consistent stochasticity is demonstrated on three different applications, namely, network calibration, adversarial robustness, and feature privacy, by boosting the performance of the respective established baselines.

==> custom_settings.tex <==

\newcommand{\PR}[1]{\textcolor{red}{\textbf{PR: #1}}}
\newcommand{\NP}[1]{\textcolor{red}{\textbf{NP: #1}}}
\definecolor{mygray}{gray}{.9}

==> figures/paper/main_teaser.tex <==
\begin{figure}[t!]
    \label{fig:main_teaser}
    \centering
    \captionsetup{font=small}
    \begin{subfigure}[b]{0.23\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{images/paper/main_graphs/classification_accuracy_main_plot.pdf}
        \vspace*{-5.5mm}
        \caption{Classification accuracy}
        \label{fig:main_teaser_accuracy}
    \end{subfigure}
    \hfill 
    %\vskip\baselineskip
    \begin{subfigure}[b]{0.23\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{images/paper/main_graphs/calibration_main_bar_plot.pdf}
        \caption{Confidence calibration}
        \label{fig:main_teaser_calibration}
    \end{subfigure}
    \hfill    
    \begin{subfigure}[b]{0.23\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{images/paper/main_graphs/adversarial_robustness_main_bar_plot.pdf}
        \caption{Adversarial robustness}
        \label{fig:main_teaser_adv_robustness}
    \end{subfigure}
    \hfill    
    \begin{subfigure}[b]{0.23\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{images/paper/main_graphs/privacy_main_bar_plot.pdf}
        \caption{Privacy preservation}
        \label{fig:main_teaser_privacy}
    \end{subfigure}
    %\caption{{\textbf{Caption}. Main caption}}
    \caption{\textbf{An overview of the effects of proposed stochastic layers in vision transformers.} The channel $j$ of every token inside the transformer's MLP block is multiplied with the same random variable $a^{j} \sim \mathcal{U}(1-\Delta,1+\Delta)$ from~\eqref{eq:noise_injection}. In~\ref{fig:main_teaser_accuracy} we see that there is no significant drop in accuracy, even when using strong stochasticity during inference. 
    Next, in~\ref{fig:main_teaser_calibration} we see that adding stochastic layers can improve network calibration, meaning that the predictive probability better depicts the uncertainty.
    In~\ref{fig:main_teaser_adv_robustness} we can see that adding stochastic layers can improve robustness against adversarial attacks.  
    Finally, in~\ref{fig:main_teaser_privacy} we see that adding stochastic layers can help with privacy preservation by reducing reconstruction quality of feature maps sent over unsecure channels.}
\end{figure}

==> figures/paper/privacy_reconstruction_uniform_everywhere.tex <==
% For CVPR 2 column format we used \begin{subfigure}[b]{0.47\columnwidth}
% and \includegraphics[width=\textwidth]{img_path}
\begin{figure}[t!]
    \centering
    \captionsetup{font=small}
    \begin{subfigure}[b]{0.47\columnwidth}
        \centering
        \includegraphics[width=0.6\columnwidth]{images/paper/privacy_reconstruction/dropout_PSNR.pdf}
        \caption{Dropout}
        \label{fig:privacy_dropout}
    \end{subfigure}
    \hfill    
    \begin{subfigure}[b]{0.47\columnwidth}
        \centering
        \includegraphics[width=0.6\columnwidth]{images/paper/privacy_reconstruction/uniform_all_dims_PSNR.pdf}
        \caption{Uniform}
        \label{fig:privacy_uniform_everywhere}
    \end{subfigure}
    \caption{{\textbf{Non-homeomorphic mappings}. Multiplying every element of the feature map $\mathcal{\Tilde{Z}}^{FC_1}_{i}$ with independent noise (e.g. Dropout~\cite{srivastava2014dropout}) is a non-homeomorphic operation, which does not preserve the privacy as well as homeomorphic stochastic layers. Dropout in~\ref{fig:privacy_dropout} matches the variance of $\mathcal{U}(0,2)$ and has a similar classification accuracy as stochastic layers with $\mathcal{U}(0.25,1.75)$. In~\ref{fig:privacy_uniform_everywhere} we compare our stochastic layers to applying independent noise everywhere.}}
    \label{fig:privacy_reconstruction_different_noise}
\end{figure}

==> figures/paper/privacy_reconstruction_uniformn.tex <==
% For CVPR 2 column format we used \begin{subfigure}[b]{0.47\columnwidth}
% and \includegraphics[width=\textwidth]{img_path}
\begin{figure}[t!]
    \centering
    \captionsetup{font=small}
    \begin{subfigure}[b]{0.23\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{images/paper/privacy_reconstruction/uniform_L1.pdf}
        \caption{$L_1$ reconstruction}
    \end{subfigure}
    \hfill    
    \begin{subfigure}[b]{0.23\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{images/paper/privacy_reconstruction/uniform_L2.pdf}
        \caption{$L_2$ reconstruction}
    \end{subfigure}
    %\vskip\baselineskip
    \begin{subfigure}[b]{0.23\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{images/paper/privacy_reconstruction/uniform_PSNR.pdf}
        \caption{PSNR reconstruction}
    \end{subfigure}
    \hfill    
    \begin{subfigure}[b]{0.23\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{images/paper/privacy_reconstruction/uniform_SSIM.pdf}
        \caption{SSIM reconstruction}
    \end{subfigure}
    
    \caption{{\textbf{Privacy preservation}. Stronger noise in our stochastic layers makes it harder to reconstruct the input from the intercepted feature map $\mathcal{\Tilde{Z}}^{FC_1}_{i}$, and privacy is better preserved.}}
    \label{fig:privacy_reconstruction_uniform}
\end{figure}

==> latex/paper/experiments_OLD.tex <==
\section{Experiments}
\label{sec:experiments}

In this section, we analyze the effect of our linear stochastic layers for vision transformers on several aspects, including classification \textbf{accuracy}, adversarial \textbf{robustness}, confidence \textbf{calibration}, and \textbf{privacy}. Furthermore, we showcase applications for \textbf{federated} and \textbf{transfer} learning, considering several image understanding tasks.
For this purpose, we will use the DeiT-S architecture~\cite{Touvron21aDeIT}. DeiT-S is one specific instance of the ViT transformer~\cite{dosovitskiy2021image} and has a parameter count and computational complexity similar to ResNet-50~\cite{He2015ResNet}.

\textbf{Training Procedure.} To explore the general behaviour of our method we use the ILSVRC-2012 ImageNet-1k dataset, which contains $1.2$M training and $50000$ validation images grouped into $1000$ classes~\cite{Russakovsky2015ImageNet}. The DeiT-S model pre-trained on ImageNet-1k is used as a starting point for all experiments, unless otherwise mentioned. All the details regarding the pre-training procedure are contained in~\cite{Touvron21aDeIT}. We insert the stochastic layer from \eqref{eq:noise_injection} into every block of the DeiT-S and fine-tune for $30$ epochs. We choose the distribution $\mathcal{P}$ as uniform $\mathcal{P} \sim \mathcal{U}(1-\Delta,1+\Delta)$. During this fine-tuning process we use the AdamW optimizer~\cite{Loshchilov2017AdamW} and a cosine scheduler with a learning rate of $10^{-5}$, which gradually decays to $10^{-6}$. We also turn off DropPath~\cite{huang2016stochasticDepth} and use the ReLU activation in order to introduce the noise to a deterministic baseline with a (piecewise) linear impact.
%We fine-tune a completely deterministic baseline as well. 
All other settings remain as in pre-training. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Effect on ImageNet Accuracy}
\label{sec:experiments_stochastic_layers}

We begin by analyzing the predictive performance of stochastic layers with regards to classification accuracy on the ImageNet validation set after fine-tuning. As presented in Figure~\ref{fig:main_teaser_accuracy}, there is no significant drop in accuracy, even when using high noise levels during inference. The network performs better if $a^{j}$ from ~\eqref{eq:noise_injection} is set to the mean of the training noise distribution $\mathbb{E}\left[\mathcal{P}\right]$ during inference. Also, the network preforms better when multiple predictions are sampled ($a^{j}\sim\mathcal{P}$, independently sampled for each block and prediction) and averaged in a Monte Carlo fashion (see Section~\ref{ssec:monte_carlo_inference} for details). However, the inference also works reasonably well when we just sample once. This is \emph{surprising} given the fact that the random variables $a^{j}$, which multiplies token channels, is sampled from a completely non-informative distribution.
The choice of noise strength and inference mode will depend on the final use-case. In the following subsections, we analyse the involved trade-offs to guide this decision.

Next, we insert the stochastic layers into the state-of-the-art Swin transformers~\cite{liu2021swin} to verify that the proposed method is not tailored for a specific ViT architecture. More precisely, we fine tune the Swin-T model, which has a parameter count and computational complexity similar to DeiT-S, following the same fine-tuning procedure as previously described. From Table~\ref{table:imnet_1k_accuracy_swin}, we observe that our stochastic layers behave well with different transformer architectures.

\input{tables/paper/classification_image_net_1k_swin}

The aim of this paper is to show the benefits of integrating proposed stochastic layers into vision transformers, with just fine-tuning and without architectural modifications. Nevertheless, we want to make sure that the training convergence is not just because of the very good initial weights. Therefore, we conduct an experiment where we train from scratch. We use 100 randomly chosen classes of the ImageNet-1k dataset. The models are trained for 300 epochs, followings the settings from~\cite{Touvron21aDeIT}. In Table~\ref{table:imnet_100_scratch_accuracy}, we see that there the networks have no problem learning with the proposed stochasticity. 

\input{tables/paper/cls_imnet_scratch_100}

\NP{Compare also to Dropout here ? and argue that ours is more severe. Also, mention local correlation and why dropout leaks information through local averaging?}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Confidence Calibration}
\label{ssec:confidence_calibration}
In practice, any inference algorithm is only useful for a decision-making system, if it can also give an indication about the confidence of its predictions. Besides good accuracy, estimating the confidence is crucial for real-world applications, where decisions have to be made with incomplete information.
%
Intuitively, if a well-calibrated classifier outputs a prediction with a confidence of $p$ (e.g. softmax score), we expect the classifier to be correct with probability $p$. 
%
It has been observed that training of complex neural networks may result in bad calibration, despite exhibiting good accuracy. Different factors, including model capacity, architecture, regularization and loss function influence the calibration quality~\cite{guo2017calibration,Minderer2021RevisitingTC}. In the following, we introduce the calibration problem in more detail, and then analyse the role of stochasticity through our experiments.

\subsubsection{Problem Definition}
We define the confidence calibration problem in the context of supervised multi-class classification, following~\cite{guo2017calibration}.   
Given the random variables $X \in \mathcal{X}$ and $Y \in \mathcal{Y}$, representing the input and labels respectively. Then a classifier $h(X)=(\hat{Y},\hat{P})$, predicting a label $\hat{Y}$ and an associated confidence $\hat{P}$, would be perfectly calibrated if
\begin{equation}
\label{eq:perfect_cal}
    \mathbb{P}(\hat{Y}=Y | \hat{P} = p) = p \quad \forall p \in \left[0,1\right].
\end{equation}

In particular, we are interested in quantifying the quality of calibration. To this end, we analyse the expected calibration error (ECE),
\begin{equation}
\label{eq:ece-org}
    \mathbb{E}_{\hat{P}}\left[\mathbb{P}(\hat{Y}=Y | \hat{P} = p) - p \right].
\end{equation}
ECE measures the expected disparity between prediction confidence and accuracy, and would be 0 in the case of~\eqref{eq:perfect_cal}.

\subsubsection{Monte Carlo Inference}
\label{ssec:monte_carlo_inference}
To achieve a good calibration, we aim to minimize the ECE~\eqref{eq:ece-org}. It has been demonstrated in the literature that model uncertainty (i.e. the posterior distribution on the network weights $w$) can be estimated using monte-carlo sampling in the context of dropout~\cite{Gal2016DropoutAA,Kendall2017WhatUD,Gal2015BayesianCN}. This way, predictions are integrated implicitly over the posterior distribution of the network weights $q(w)$ as,
\begin{equation}
\label{eq:mc-inference}
    p(y|x) \approx \int p(y | x, w) q(w) dw \approx \frac{1}{T} \sum_{t=1}^{T} p(y| x, \hat{w}_t),
\end{equation}
approximated by T samples $\hat{w}_t$~\cite{Gal2015BayesianCN}, generated by applying dropout at test time.
Since our stochastic layers naturally offer such sampling for vision transformers, our goal is to investigate their effect on network calibration when performing inference with ~\eqref{eq:mc-inference}.

\subsubsection{Calibration Experiments}
\textbf{Evaluation Metric.}
To estimate~\eqref{eq:ece-org} using finite samples,~\cite{Naeini2015ObtainingWC} sorts network predictions $\hat{P}$ into $M$ equidistant bins.
With $B_m$ denoting the indices of all samples in the interval $\left(\frac{m-1}{M},\frac{m}{M}\right]$, we compute the accuracy and confidence for each bin as, 
\begin{align}
\label{eq:ece-bins}
    &\text{acc}(B_m) = \frac{1}{|B_m|}\sum_{i \in B_m} \mathbf{1}(\hat{y}_i=y_i), \\
    &\text{conf}(B_m) = \frac{1}{|B_m|}\sum_{i \in B_m} \hat{p}_i.
\end{align}
Then the ECE is approximated by computing the disparity between accuracy and confidence for samples from each bin as,
\begin{equation}
\label{eq:ece-finite}
    \text{ECE} = \sum_{m=1}^{M}\frac{|B_m|}{n} \left|\text{acc}(B_m) - \text{conf}(B_m)\right|.
\end{equation}
For our experiments, we compare the ECE with $M=15$ bins ~\cite{guo2017calibration} on the ImageNet-1k validation set.

\noindent\textbf{Setup.} We evaluate the calibration of vision transformers with and without stochastic layers, using models from Section~\ref{sec:experiments_stochastic_layers}. As a baseline we compare to our deterministic model, as well as to Monte Carlo dropout~\cite{Gal2016DropoutAA}, which is a strong baseline for uncertainty estimation. To this end, we replace our stochastic layers with dropout. To create a fair counterpart for our model with a noise level $\Delta$, we choose the dropout probability $p$ such that its underlying Bernoulli distribution matches the variance of the distribution $\mathcal{P}$ from~\eqref{eq:noise_injection}. The strongest baseline would be to use model ensembles~\cite{lakshminarayanan2017ensambleUncertanity}. However, we do not include ensembles due to the computational demand on big datasets, which also limits the practical application. On the other hand, a very simple and effective technique to improve confidence calibration is given by softmax temperature tuning~\cite{guo2017calibration}. Very recently, this has been also shown to work well with transformer architectures~\cite{Minderer2021RevisitingTC}. We use it in our experiments, since it can be simply applied to the baselines and our models during evaluation.

\input{tables/paper/calibration}
\noindent\textbf{Results.} The results are summarized in Table~\ref{table:calibration_results}. Compared to the baseline, temperature scaling~\cite{guo2017calibration} improves the calibration quality. The best results however are achieved in combination with our approach, through Monte Carlo sampling and confidence estimation. Calibration accuracy tends to improve with higher number of samples.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Adversarial Robustness}
\label{sec:adversarial_robustness}
Besides the accuracy and privacy, another important aspect of the network is its behaviour with respect to adversarial samples~\cite{Szegedy2014IntriguingPO}. If we are interested to design algorithms that use visual features which resemble the human perception, then small adversarial perturbations in the pixel intensities of the input image must not lead to different decisions in the output~\cite{Ilyas2019AdversarialEA}. Also, we want to avoid exposition of such vulnerabilities to actors with malintent. We therefore desire networks that are adversarially robust~\cite{Goodfellow2015ExplainingAH}. 

\textbf{Adversarial Attacks.}
In general, adversarial attacks exploit the differentiability of the network $h(x)$ and its prediction loss $\mathcal{L}(h(x))$ with respect to the input image $x$. Given a desired target label $t$, the attack aims to slightly pertubate the input $x$ to maximize the prediction score for label $l$.

For instance, the Fast Gradient Sign Method (FGSM)~\cite{Szegedy2014IntriguingPO} forges an adversarial sample $\hat{x}$ by applying,
\begin{equation}
\label{eq:fgsm}
    \hat{x} = x + \epsilon \, \text{sgn}(\nabla_x \mathcal{L}(h(x), l)),
\end{equation}
where $\epsilon$ is a bound that determines the attack strength (and the visibility of the perturbation).

To craft stronger adversarial samples, \eqref{eq:fgsm} is repeated multiple times with step size $\alpha$, followed by a projection to an $\epsilon$ hypercube around the initial sample $x$,
\begin{equation}
\label{eq:pgd}
    \hat{x}^{k} = \Pi_{\epsilon} \left[x^{k-1} + \alpha \, \text{sgn}(\nabla_x \mathcal{L}(h(\hat{x}^{k-1}), l))\right],
\end{equation}
known as the projected gradient descent (PGD) attack~\cite{Madry2018TowardsDL}. 

\textbf{Adversarial Defenses.}
Numerous approaches have been proposed in the literature to defend against such attacks, which we roughly categorized into adversarial training~\cite{Kurakin2017AdversarialML,Shafahi2019AdversarialTF,Wong2020FastIB,Zhang2019TheoreticallyPT,Madry2018TowardsDL}, certified defenses~\cite{Cohen2019CertifiedAR,Croce2019ProvableRO,Zhai2020MACERAA,Salman2019ProvablyRD}, regularization~\cite{Ciss2017ParsevalNI,Ross2018ImprovingTA,Finlay2019ScaleableIG,Ororbia2016UnifyingAT,Jakubovitz2018ImprovingDR,Gu2015TowardsDN}, and gradient obfuscation~\cite{46641,Pinot2019TheoreticalEF,Rakin2019ParametricNI,Lee2021GradDivAR}.
%
In particular,~\cite{Pinot2019TheoreticalEF,Rakin2019ParametricNI,Lee2021GradDivAR} show that injection of stochasticity into the network improve adversarial robustness. In that line, our goal is to investigate the impact of our stochastic layers with regards to the adversarial robustness of the network.

\input{tables/paper/adversarial_robustness}

\subsubsection{Robustness Experiments}

\noindent\textbf{Setup.} In order to evaluate adversarial robustness, we craft adversarial examples for each image in the ImageNet-1k validation set, and test the model's accuracy on those adversarial examples. We do this by using the PGD attack~\eqref{eq:pgd} with $10$ iterations (PGD-10). When crafting each adversarial example, we initialize the attack's starting point randomly inside the $\epsilon-$hypercube and restart this procedure $5$ times to find the strongest attack, following the standard benchmark of~\cite{Wong2020FastIB,Shafahi2019AdversarialTF}. We test for two different $\epsilon-$hypercube constraints $\epsilon= \{ 2, 4\}$. The attack step $\alpha$ from~\eqref{eq:pgd} is $1$ in both cases.

\noindent\textbf{Results with Adversarial Training.} First, we test the effect of our stochastic layers combined with adversarial robustness training. We take the same DeiT-S starting point as described in Section~\ref{sec:experiments_stochastic_layers} and additionally use adversarial training while fine-tuning the inserted stochastic layers. More specifically, we use the efficient adversarial training described in~\cite{Wong2020FastIB}. 
Adversarial training of~\cite{Wong2020FastIB} is an effective remedy for adversarial vulnerability, and in fits in our standard training protocol~\cite{Athalye2018ObfuscatedGG,Madry2018TowardsDL} without much overhead.
%We do this because adversarial training has been shown to be truly effective in circumventing adversarial vulnerability and it also fits in the standard training protocol~\cite{Athalye2018ObfuscatedGG,Madry2018TowardsDL}.
The baseline is a deterministic model fine-tuned with adversarial training. During this fine-tuning process regular hyperparameters remain the same as in Section~\ref{sec:experiments_stochastic_layers}, except for using $20$ epochs now. The adversarial training hyper-parameters are as above, except for the step sizes which are $\alpha= \{2.5, 5.0 \}$ for $\epsilon= \{ 2, 4\}$ respectively. In Table~\ref{tab:adv_robustness_robust_tr} we see that adding stochastic layers improves adversarial robustness beyond adversarial training. This effect is stronger if the networks are sampled in a Monte Carlo fashion. Also, while sampling, the clean accuracy becomes higher than in the baseline. This is particularly interesting, since it has been shown that there is a trade-off between between adversarial robustness and clean accuracy~\cite{Zhang2019TheoreticallyPT}.

\noindent\textbf{Results without Adversarial Training.} We also test the robustness of our stochastic layers without adversarial training. For this experiment we take the models trained in Section~\ref{sec:experiments_stochastic_layers} and evaluate the robustness. In Table~\ref{tab:adv_robustness_raw} we first notice that the baseline has no adversarial robustness, like it has been observed in literature~\cite{Shafahi2019AdversarialTF}. We also notice that our stochastic layer achieves a significant level of robustness, even without adversarial training. Robustness becomes stronger as the strength of the stochasticity increases. We also observe that clean accuracy in our method can be largely recovered through Monte Carlo inference, especially in the case of high noise. For $\Delta=1.0$, the clean accuracy improves from $72.93\% \rightarrow 77.75\%$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Privacy-preserving Features}
\label{ssec:private_features}
Sharing image features is an important part of collaborative systems that distribute computations across nodes. 
Applications include camera localization~\cite{Speciale2019PrivacyPI}, structure-from-motion~\cite{Geppert2020PrivacyPS} in a shared environment, federated learning~\cite{bonawitz2019towards,kairouz2019advances,Konecn2016FederatedLS}, or split learning/inference~\cite{gupta2018distributed,vepakomma2018split}.
%
To address privacy issues, problem-specific solutions have been proposed. ~\cite{Speciale2019PrivacyPI,Geppert2020PrivacyPS} obfuscate the geometry to maintain privacy of sparse features~\cite{Pittaluga2019RevealingSB}. Homomorphic encryption guarantee privacy in the context of feature extraction~\cite{Qin2014TowardsEP,Hsu2012ImageFE}, retrieval~\cite{Engelsma2020HERSHE}, and federated learning~\cite{Fang2021PrivacyPM}. However, these methods do not readily extend to many practical cases of distributed learning. This includes split learning~\cite{gupta2018distributed,vepakomma2018split} where features of the data are shared, after being processed by a part of the complete network.
%The local network could be a generic visual feature extractor that may also be trained. The top part of the network on the other hand is then processed on a centralized server, without sharing the original images. In similar fashion, one could split the workload for inference across different devices, e.g. across a mobile device and a server.
Even though the feature extraction removes information from the input image, it is still possible reconstruct the input~\cite{Ulyanov2018DeepIP,Zhang2020TheSR,Yin2020DreamingTD,Wang2021IMAGINEIS} or privacy-related attributes thereof~\cite{Basu2019MembershipMI,Singh2021DISCODA}.

In Section~\ref{ssec:input_reconstruction} we first analyse to which extent vision transformers preserve the privacy of features. To this end, we train a decoder to reconstruct the input from features of different transformer blocks, and show the impact of our stochastic layers on reconstruction quality, 
%sample complexity of the reconstruction problem, 
and quantify the trade-off between accuracy and noise level.
In Section~\ref{ssec:private_federate_learning} we further demonstrate that the stochastic network still retains its generalization ability and flexibility to transfer to other datasets, and is therefore a directly applicable for federated learning, while ensuring a higher level of privacy. 
%\textcolor{red}{ This subsection looks poor due to the lack  or too much of fragmentation.}

\subsubsection{Input Image Reconstruction}
\label{ssec:input_reconstruction}
We now analyse the models introduced in Section~\ref{sec:experiments_stochastic_layers} with regards to feature privacy. To simulate a distributed learning environment, we split the model into two parts. The local network is the part of the network which processes the input up until the feature map $\mathcal{\Tilde{Z}}^{FC_1}_{i}$ from~\eqref{eq:noise_injection} in block $i$ . It then sends $\mathcal{\Tilde{Z}}^{FC_1}_{i}$ to the centralized server where it is processed by the second part of the network.

\noindent\textbf{Threat Model.} The adversary intercepts feature maps $\mathcal{\Tilde{Z}}^{FC_1}_{i}$, while they are being sent to the server. Similarly, an adversary could potentially obtain a small amount of input images corresponding to the sent feature maps and use them to learn a model which reconstructs the input image. When a new feature map $\mathcal{\Tilde{Z}}^{FC_1}_{i}$ is sent to the server, the adversary is now able to reconstruct the corresponding input image and thus violate the users privacy.

\noindent\textbf{Decoder Attack.} We train a decoder to reconstruct the input image from the feature map $\mathcal{\Tilde{Z}}^{FC_1}_{i}$. The decoder is an enhanced version of the decoder used in~\cite{isola2018imagetoimage}. We use the $L_1$ reconstruction loss for training and we train it on a small subset of the ImageNet-1k dataset, containing $20$ randomly chosen classes. We evaluate the reconstruction quality by measuring the difference of the reconstructed and the input image using the $L_1$, $L_2$, peak signal to noise ratio (PSNR) and structural similarity index measure (SSIM) metrics.

\input{figures/paper/privacy_reconstruction_uniformn}
\input{figures/paper/privacy_reconstruction_uniform_everywhere}

\noindent\textbf{Results.} From Figure~\ref{fig:privacy_reconstruction_uniform} we conclude that it is harder to reconstruct the input from feature maps $\mathcal{\Tilde{Z}}^{FC_1}_{i}$ at depth $i$, when using stochastic layers. The gap to the deterministic network increases with stronger levels of noise. Next, in Figure~\ref{fig:privacy_reconstruction_different_noise} we compare our stochastic layers with a non-homeomorphic mapping, which multiplies every element of $\mathcal{\Tilde{Z}}^{FC_1}_{i}$ from~\eqref{eq:noise_injection} with a different random variable. We see that its reconstruction quality is close to the deterministic baseline, offering less privacy than our approach.

\subsubsection{Privacy-preserving Federated Learning}
\label{ssec:private_federate_learning}

To simulate a federated learning setup, we take the models from the privacy experiments in Section~\ref{ssec:private_features}, and freeze the encoders which produce the feature map $\mathcal{\Tilde{Z}}^{FC_1}_{i}$. An encoder now represents the model on a decentralized device. We then perform federated learning by sending feature maps $\mathcal{\Tilde{Z}}^{FC_1}_{i}$ (instead of sending the input images, which should remain private) to the centralized server, in order to learn a new task.  We train a small classifier for each model on the CIFAR10/100~\cite{Krizhevsky2009LearningML} datasets. The classifier contains $2$ fully connected layers, followed by a softmax layer.

\noindent\textbf{Results.} In Figure~\ref{fig:privacy_federated_learning} we visualize the trade-off between the accuracy on the new tasks and the input reconstruction. We observe that using stochastic layers offers better privacy in this setting at a cost of task performance. With this knowledge one can choose a trade-off point, in accordance with the final task and use-case.

\input{figures/paper/privacy_federated_learning}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Transfer Learning}
\label{sec:transfer_learning}
Transfer learning is concerned with the problem of leveraging information from a rich source domain (with large labeled datasets), in order to improve the learning on a different downstream task, for which only limited data is available~\cite{Donahue2014DeCAFAD,Razavian2014CNNFO}.
For vision problems, the ImageNet~\cite{Russakovsky2015ImageNet}-trained models are established starting points for the transfer learning on natural images, due to the large variability and scale of the dataset.

\noindent\textbf{Setup.} We compare transferability of our features on a standard benchmark suite containing the aircraft~\cite{maji13fine-grained}, birdsnap~\cite{Berg2014BirdsnapLF}, CIFAR10/100~\cite{Krizhevsky2009LearningML}, Caltech-101~\cite{FeiFei2004LearningGV}, Caltech-256~\cite{Griffin2007Caltech256OC}, cars~\cite{Krause2013CollectingAL}, DTD~\cite{Cimpoi2014DescribingTI}, flowers~\cite{Nilsback2008AutomatedFC}, food-101~\cite{Bossard2014Food101M}, pets~\cite{Parkhi2012CatsAD}, and SUN-397~\cite{Xiao2010SUNDL} datasets. We follow the setup of~\cite{salman2020adveTransfer}. We use the AdamW optimizer~\cite{Loshchilov2017AdamW} with an inital learning rate of $10^{-5}$ and weight decay of $5\times10^{-2}$. The transfer learning lasts for $150$ epochs and the learning rate gets decayed by a factor of $10$ every $50$ epochs.

\input{tables/paper/transfer_learning}

\noindent\textbf{Results.} Our findings are summarized in Table~\ref{table:transfer_learning}. Despite the tendency of big transformer architectures to quickly overfit, all compared method obtain competitive results. We observe that our stochastic networks are able to retain their performance and sometimes even exceed the deterministic baseline. The results are quite robust to the level of noise applied. We therefore conclude that the transferability is not negatively impacted by introducing the stochasticity.


% One step closer to binarization/compression (with results)












\newcommand{\PR}[1]{\textcolor{red}{\textbf{PR: #1}}}
\newcommand{\NP}[1]{\textcolor{red}{\textbf{NP: #1}}}
\definecolor{mygray}{gray}{.9}

==> tables/paper/classification_image_net_1k_swin.tex <==
\begin{table}[t!]
\centering
\tableFont
\captionsetup{font=small}
\caption{{\textbf{ImageNet-1k classification accuracy with different vision transformer architectures}. Stochastic layers perform well with different architectures.}}

%\begin{adjustbox}{\columnwidth}
%\renewcommand\arraystretch{1}
%\resizebox{0.7\columnwidth}{!}{
\begin{tabular}{|l|l|c|c|c|}
\hline
\multicolumn{2}{|c|}{} & \multicolumn{3}{c|}{Accuracy$\uparrow$}  \\ \cline{3-5}
\multicolumn{2}{|c|}{} & $\Delta=0$  & $N=1$ & $N=50$         \\ \hline \hline
\multirow{4}{*}{DeiT-S~\cite{Touvron21aDeIT}} 
 & Regular              & $79.61\%$ & $79.61\%$ & $79.61\%$ \\ \cline{2-5}
 & $\Delta=0.1$         & $79.83\%$ & $79.58\%$ & $79.86\%$ \\ \cline{2-5}
 & $\Delta=0.5$         & $79.60\%$ & $77.43\%$ & $79.72\%$ \\ \cline{2-5}
 & $\Delta=1.0$         & $77.96\%$ & $72.93\%$ & $77.75\%$ \\ \hline \hline 
\multirow{4}{*}{Swin-T~\cite{liu2021swin}} 
 & Regular              & $81.03\%$ & $81.03\%$ & $81.03\%$ \\ \cline{2-5}
 & $\Delta=0.1$         & $81.02\%$ & $81.02\%$ & $81.09\%$ \\ \cline{2-5}
 & $\Delta=0.5$         & $81.05\%$ & $79.40\%$ & $81.07\%$ \\ \cline{2-5}
 & $\Delta=1.0$         & $80.20\%$ & $75.95\%$ & $80.08\%$ \\ \hline 
 
\end{tabular}
%}
\label{table:imnet_1k_accuracy_swin}
\end{table}

% \multirow{2}{*}{\makecell{Regular}} 
%  & DeiT-S~\cite{Touvron21aDeIT}         & $79.61\%$ & $79.61\%$ & $79.61\%$ \\ \cline{2-5}
%  & Swin-T~\cite{liu2021swin}         & $81.03\%$ & $81.03\%$ & $81.03\%$ \\ \hline \hline
% \multirow{2}{*}{\makecell{$\Delta=0.1$}} 
%  & DeiT-S~\cite{Touvron21aDeIT}         & $79.83\%$ & $79.58\%$ & $79.86\%$ \\ \cline{2-5}
%  & Swin-T~\cite{liu2021swin}         & $81.02\%$ & $81.02\%$ & $81.09\%$ \\ \hline \hline
% \multirow{2}{*}{\makecell{$\Delta=0.5$}} 
%  & DeiT-S~\cite{Touvron21aDeIT}         & $79.60\%$ & $77.43\%$ & $79.72\%$ \\ \cline{2-5}
%  & Swin-T~\cite{liu2021swin}         & $81.05\%$ & $79.40\%$ & $81.07\%$ \\ \hline \hline
% \multirow{2}{*}{\makecell{$\Delta=1.0$}} 
%  & DeiT-S~\cite{Touvron21aDeIT}         & $77.96\%$ & $72.93\%$ & $77.75\%$ \\ \cline{2-5}
%  & Swin-T~\cite{liu2021swin}         & $80.20\%$ & $75.95\%$ & $80.08\%$ \\ \hline 
 

==> tables/paper/cls_imnet_scratch_100.tex <==
\begin{table}[t!]
\centering
\tableFont
\captionsetup{font=small}
\caption{{\textbf{ImageNet-100 classification accuracy from scratch}. The networks have been successfully trained from scratch on $100$ randomly chosen classes of the ImageNet-1k dataset.}}
%\begin{adjustbox}{\columnwidth}
%\renewcommand\arraystretch{1}
%\resizebox{0.7\columnwidth}{!}{
\begin{tabular}{|l|l|c|c|c|}
\hline
\multicolumn{2}{|c|}{} & \multicolumn{3}{c|}{Accuracy$\uparrow$}  \\ \cline{3-5}
\multicolumn{2}{|c|}{} & $\Delta=0$  & $N=1$ & $N=50$         \\ \hline \hline

\multicolumn{2}{|l|}{Regular}  & $89.18\%$ & $89.18\%$ & $89.18\%$  \\ \hline 

\multicolumn{2}{|l|}{$\Delta=0.1$}                       & $89.40\%$ & $89.30\%$ & $89.28\%$  \\ \hline 

\multicolumn{2}{|l|}{$\Delta=0.5$}                       & $89.48\%$ & $88.58\%$ & $89.48\%$  \\ \hline 

\multicolumn{2}{|l|}{$\Delta=1.0$}                       & $89.06\%$ & $88.00\%$ & $89.24\%$  \\ \hline

\end{tabular}
%}
\label{table:imnet_100_scratch_accuracy}
\end{table}
